CCO-VOXEL: Chance Constrained Optimization over Uncertain Voxel-Grid Representation for Safe Trajectory Planning

We present CCO-VOXEL: the very first chance-constrained optimization (CCO) algorithm that can compute trajectory plans with probabilistic safety guarantees in real-time directly on the voxel-grid representation of the world. CCO-VOXEL maps the distribution over the distance to the closest obstacle to a distribution over collision-constraint violation and computes an optimal trajectory that minimizes the violation probability. Importantly, unlike existing works, we never assume the nature of the sensor uncertainty or the probability distribution of the resulting collision-constraint violations. We leverage the notion of Hilbert Space embedding of distributions and Maximum Mean Discrepancy (MMD) to compute a tractable surrogate for the original chance-constrained optimization problem and employ a combination of A* based graph-search and Cross-Entropy Method for obtaining its minimum. We show tangible performance gain in terms of collision avoidance and trajectory smoothness as a consequence of our probabilistic formulation vis a vis state-of-the-art planning methods that do not account for such nonparametric noise. Finally, we also show how a combination of low-dimensional feature embedding and pre-caching of Kernel Matrices of MMD allows us to achieve real-time performance in simulations as well as in implementations on on-board commodity hardware that controls the quadrotor flight

==> method_arun.tex <==
\subsection{ Noise Analysis}

\subsubsection{Experimental Setup}

\subsubsection{Noise Model}



\subsection{MMD Computation}

\begin{tabular}{|c|c|}
\hline
  $\delta$   & Dirac function \\
  \hline
    $P^{des}$ &  Desired distribution \\
    \hline
    f(.) & Distance function \\
    \hline
    $\mu$ & RKHS embedding of the actual distribution \\
    \hline
    $\mu^{des}$ & RKHS embedding of the desired distribution \\
    \hline
    $\eta$ & Chance constrain value \\ 
    \hline 
    K( .,. ) & Kernel function \\
    \hline
    $d_{i}$ & $i^{th}$ sample in the distance distribution \\
    \hline
    $r_{safe}$ & Safe radius of UAV \\
    \hline 
\end{tabular}

\subsubsection{Problem Formulation}

 \begin{subequations} \label{CCO}
 \begin{align}
    E(C_{i}) = \sum_{ i=0 }^{N} \lambda_{1} MMD(C_{i}) + \lambda_{2} F_{a}(C_{i}) + \lambda_{3} \lVert C_{i-1} - 2C_{i} + C_{i+1} \lVert 
 \end{align}
    \begin{align}
   \textrm{s.t.} \quad   P( (r_{safe} - d_{i } ) < 0 ) >  \eta   
    \end{align}
 \end{subequations}
 
 \[  F_{a}(C_{i}) = ( a_{min} - a_{c_i} )(a_{max} - a_{c_i} ) \]
Optimization of functions using constrains in the form of  \ref{CCO} is known as Chance Constrained Optimization (CCO). In general CCO has a high computational complexity that  stems from the presence of chance constrains, a  non linear function \textit{f(.)} and a large set of samples . In this section we reformulate this problem into a tractable non linear optimization problem.  \par

Our solution is based on the theorems proposed in \cite{Reactive_navigation_RKHS}, where it states that MMD can act as a surrogate to the moment matching problem and decreasing the Maximum Mean Discrepancy (MMD) residual between the RKHS embedding of $\mathnormal{P_{f}}$ and desired distribution $\mathnormal{P_{f^{des}}}$, is a method to match the first \textit{d} moments between the distributions. 
\begin{equation} \label{MMD}
L_{dist}    = \lVert \mu_{P_{f}} - \mu_{P^{des}} \lVert^{2}  
\end{equation}

Equation \ref{MMD} can be further expanded to obtain 

\begin{equation} \label{MMD_expand}
    \lVert \mu - \mu_{des} \lVert ^{2} = \langle \boldsymbol{\mu_{P_{f}}} , \boldsymbol{ \mu_{P_{f}} }\rangle - 2 \langle \boldsymbol{ \mu_{P_{f}}}, \boldsymbol{\mu_{P^{des}}}  \rangle + \langle \boldsymbol{\mu_{P^{des}}}  , \boldsymbol{\mu_{P^{des}}}  \rangle 
\end{equation}

Equation \ref{MMD_expand} computes the inner product between the functions, that are linear combinations of kernel functions.  The use of the "kernel trick" allows for the computation of the inner product by pointwise computation of the kernel function. 


\subsubsection{Desired Distribution}

In general construction of an exact desired distribution is an intractable problem \cite{Reactive_navigation_RKHS} , therefore we propose a unique representation of the desired distribution as a dirac function. Furthermore, this representation provides attractive properties which leverages computational advantages. \par

Consider a distance distribution $\mathnormal{Q}$ represented by samples \textit{$\Tilde{d_{i}}$}. The distribution can be considered ideal if all the samples in it are avoiding the obstacle i.e $\forall \Tilde{d_{i}} \in \mathnormal{Q}$, $r_{safe} -\Tilde{d_{i}} < 0 $.   \par

\begin{equation} \label{dirac}
f(d_{i}) = \max ( 0 , (r_{safe} - \Tilde{d_{i}} )) 
\end{equation}
\[ \forall \Tilde{d_{i}} \in \mathnormal{Q}\]

Through equation \ref{dirac} where all samples are drawn from an ideal distribution we observe that $f(d_{i})$ is a set of zeros. {\color{blue}{\textbf{To be Continued}}}

\begin{equation}
     P(f(d)) \rightarrow \delta
\end{equation}


\subsubsection{Computing MMD through Kernel Matrices}

Let ${d_{0} ,d_{0} , d_{1}, d_{2} , ... , d_{n}}$ be the samples drawn from the distance distribution $\mathnormal{P}$, the kernel mean function can be used to represent this distribution in the RKHS space as given in equation  \ref{kernel_mean}, where $\alpha$ is the weight vector that describes the weight of individual sample and $f(d_{i})$ is given by equation \label{dirac}. 


\begin{equation} \label{kernel_mean}
   \mu = \sum_{i=0}^{N} \alpha_{i}k( f(d_{i}) , .) 
\end{equation}

Considering the desired distribution as the dirac function $(\mu_{des} = \delta)$ and substituting in equation \ref{MMD} we get \ref{MMD_substituted}. 

% \begin{equation} \label{MMD_substituted}
%   L_{dist} = \lVert \mu - \delta \lVert ^{2}
% \end{equation}

\begin{subequations} \label{MMD_substituted} 
\begin{equation}
   L_{dist} = \lVert \mu - \delta \lVert ^{2}
\end{equation}    
\begin{equation}
\lVert \mu - \delta \lVert ^{2} = \langle \boldsymbol{\mu(d)} , \boldsymbol{\mu(d)} \rangle - 2 \langle \boldsymbol{\mu(d)}, \boldsymbol{\delta} \rangle + \langle \boldsymbol{\delta} , \boldsymbol{\delta} \rangle
\end{equation}
\end{subequations}

By substituting equation \ref{kernel_mean} in \ref{MMD_substituted} we obtain equation \ref{MMD_main}


\begin{subequations} \label{MMD_main} 
\begin{equation}
  \langle \boldsymbol{ \mu(d)} , \boldsymbol{\mu(d)} \rangle = \langle  \sum_{i=0}^{N} \alpha_{i} \boldsymbol{ K( f(d_{i}) , .)} , \sum_{i=0}^{N} \alpha_{i} \boldsymbol{ K( f(d_{i}) , .)} \rangle 
\end{equation}    
\begin{equation}
\langle \boldsymbol{ \mu(d) , \delta } \rangle = \langle \sum_{i=0}^{N} \alpha_{i} \boldsymbol{ K( f(d_{i}) , .)}  , \sum_{i=0}^{N} \beta_{i} \boldsymbol{ K( \delta , .)} \rangle 
\end{equation}
\begin{equation}
   \langle \boldsymbol{ \delta , \delta} \rangle = \langle \sum_{i=0}^{N} \beta_{i} \boldsymbol{K(\delta , .)}  , \sum_{i=0}^{N} \beta_{i} \boldsymbol{K(\delta , .)} \rangle  
\end{equation}
\end{subequations}

Using the kernel trick on equation \ref{MMD_main} we can reduce the function to 

\begin{equation}
    \lVert \mu - \delta \lVert ^{2} = \mathbf{C_{\alpha}K_{ff}C_{\alpha}^{T} - 2 C_{\alpha}K_{f\delta}C_{\psi}^{T} + C_{\psi}K_{\delta\delta}C_{\psi}^{T} } 
\end{equation}

where $\boldsymbol{\alpha}$ , $\boldsymbol{\psi}$ are the weight vectors    

\[ \mathbf{C_{\alpha}} =   \begin{bmatrix}
\alpha_{0} , \alpha_{1} , ... , \alpha_{n} 
\end{bmatrix} \]

\[ \mathbf{C_{\psi}} =   \begin{bmatrix}
\psi_{0} , \psi_{1} , ... , \psi_{n} 
\end{bmatrix} \]

\[ \mathbf{K_{ff}} = \begin{bmatrix}
k( f(d_{0}) , f(d_{0})  & \hdots & k( f(d_{0}) , f(d_{n}) \\
k( f(d_{1}) , f(d_{0})  & \hdots & k( f(d_{1}) , f(d_{n}) \\
\vdots                  & \ddots    & \hdots & \\ 
k( f(d_{n}) , f(d_{0})  & \hdots & k( f(d_{n}) , f(d_{n}) \\
\end{bmatrix} \]


\[ \mathbf{K_{f\delta}} = \begin{bmatrix}
k( f(d_{0}) , \delta(f(d_{0})) & \hdots & k( f(d_{0}) , \delta(f(d_{n})) \\
k( f(d_{1}) , \delta(f(d_{0})) &  \hdots & k( f(d_{1}) ,\delta( f(d_{n})) \\
\vdots                  & \ddots    & \hdots & \\ 
k( f(d_{n}) ,\delta( f(d_{0})) &  \hdots & k( f(d_{n}) , \delta(f(d_{n})) \\
\end{bmatrix} \]

\[ \mathbf{K_{f\delta}} = \begin{bmatrix}
k( \delta(f(d_{0})) , \delta(f(d_{0})) &  \hdots & k( \delta(f(d_{0})) , \delta(f(d_{n})) \\
k( \delta(f(d_{1})) , \delta(f(d_{0})) &  \hdots & k(\delta(f(d_{1})) ,\delta( f(d_{n}))) \\
\vdots                  & \ddots    & \hdots & \\ 
k(\delta(f(d_{n})) , \delta(f(d_{0}))) &  \hdots & k(\delta(f(d_{n})) , \delta(f(d_{n})))) \\
\end{bmatrix} \]


\subsubsection{Feature space embedding of distance measurements}
Although RKHS allows for direct embedding of samples from the distributions $\mathbf{P_{f}}$ and $\delta$, the presence of large number of samples would create high dimensional matrices which would increase the computation time. A workaround is to create in intermediate feature space representation for the distributions and compute the MMD cost for the samples in the feature space. \par    

An autoencoder is used to efficiently learn the feature space representation of the distribution. The goal is to determine an appropriate encoder \textit{$W_{1}$} and decoder \textit{$W_{2}$} pair such that they perform an identity operation.  The training is performed by optimizing the loss function given in equation \ref{autoencoder:a}. The training data consists of $\mathnormal{n}$  distributions each with $\mathnormal{m}$ samples, the data matrix $\boldsymbol{P}$ is of dimension $\boldsymbol{R^{m \times n }}$, the matrix \textit{$W_{1}$} is used to encode the high dimensional distribution data to a low dimension feature output is of dimension $\boldsymbol{R^{n \times p }}$ where $p <n$. The decoder \textit{$W_{2}$}  is further trained to re-construct the distribution from the feature vector.  


 \begin{subequations} \label{autoencoder}
    \begin{align}
       \min_{ \boldsymbol{ W_{1}} ,\boldsymbol{ W_{2}}} \lVert \boldsymbol{PW_{1}W_{2} - P} \lVert^{2} \label{autoencoder:a} \\ 
        \boldsymbol{ D = PW_{1} } \label{autoencoder:b}
    \end{align}
 \end{subequations}
 
 During implementation the distance distribution $\mathnormal{P}$ is encoded into a feature space representation $\mathnormal{D}$ and is used in the MMD formulation.
 

\subsection{Initial Path Searching}

The initial path searching algorithm searches for a collision free and dynamically feasible trajectory that is optimal over control cost and time. The proposed front end path searching algorithm is built upon kinodynamic A* algorithm which was proposed in  \cite{FastPlanner}.   {\color{blue}{\textbf{To be Continued}}}


\[ \Delta M  = M_{i=1} - M_{i}  \] 
\[ e_{c} = ( \lVert u \lVert^{2} + \rho )\tau + \Delta M  + h  \]


\subsection{Trajectory Optimization}

\subsubsection{ Trajectory Formulation as Bernstein Polynomial}

The Bernstein polynomial is defined as :

 \begin{subequations} \label{bernstein}
    \begin{align}
        b_{i}^{n} = {n\choose i}t^{i}(1-t)^{n-i} \\ 
         B(t) = \sum_{i=0}^{10} \mathnormal{c_{i}} b_{n}^{i}
    \end{align}
 \end{subequations}
 
Where \mathnormal{n} is the degree of the Bernstein polynomial $\mathnormal{B(t)}$, $n\choose i$ is the binomial coefficient, and $\mathnormal{c_{i}}$ are the coefficients that fit the Bernstein polynomial to the given waypoints.   \par

To obtain the set of coefficients that fit the given trajectory we formulate it as a quadratic programming problem. The trajectory $x_{t_i}$ and its derivatives are parameterized  in the following form.   


\begin{center}
     $\boldsymbol{Pc_{\mu}} = \begin{bmatrix} {x_{t_{0}} }\\
                            {x_{t_{1}} }\\
                            \vdots \\ 
                            {x_{t_{f}} }
                \end{bmatrix}
            $
    ;  $\boldsymbol{\dot{P}c_{\mu}}= \begin{bmatrix} {\dot{ x}_{t_{0}} }\\
                            { \dot{x}_{t_{1}} }\\
                            \vdots \\ 
                            {\dot{x}_{t_{f}} }
                \end{bmatrix}
            $
    and  $\boldsymbol{\ddot{P}c_{\mu}}= \begin{bmatrix} {\ddot{ x}_{t_{0}} }\\
                            { \ddot{x}_{t_{1}} }\\
                            \vdots \\ 
                            {\ddot{x}_{t_{f}} }
                \end{bmatrix}
            $
\end{center}


Where the matrix \mathnormal{P} is the time independent basis function and $\mathbf{c_{\mu}}$ is the coefficient vector.   

\begin{subequations}
   \begin{align}
       \min \boldsymbol{c_{\mu}}\mathbf{P^{T}}\mathbf{P}\boldsymbol{c_{\mu}} - c_{\mu}\mathbf{x_{\mu}} \\
       \mathbf{A_{eq}}\mathbf{c_{\mu}} = \mathbf{b_{eq}}
   \end{align}
\end{subequations}

Where the matrices $\boldsymbol{A_{eq}}$ is obtained by stacking the first and last rows of $\boldsymbol{P}$ and its derivatives. The matrix $\boldsymbol{b_{eq}}$ is obtained by stacking the initial and final position, velocity and acceleration.   



\begin{center}
     $\mathbf{A_{eq}} =  
\begin{bmatrix}
P_{0} \\
\dot{P_{0}} \\ 
\ddot{ P_{0}} \\
P_{f} \\
\dot{P_{f}} \\ 
\ddot{ P_{f}} \\
\end{bmatrix}
            $
            $  \mathbf{b_{eq}} = \begin{bmatrix}
            x_{t_{0}} \\ 
            \dot{x}_{t_{0}} \\
            \ddot{x}_{t_{0}} \\
            x_{t_{f}} \\
            \dot{x}_{t_{f}} \\
            \ddot{x}_{t_{f}}
            \end{bmatrix} $
\end{center}

As explained in \cite{linerize_bernstein} we reduce the optimization problem to linear equations 

\begin{center}
       $\left[
\begin{array}{c|c}
P^{T}P & A \\
\hline
A^{T} & 0_{6 \times 6}
\end{array}
\right] \boldsymbol{c}_{\mu} $ = \begin{bmatrix}
\mathbf{P}^{T}x_{\mu} \\
b_{eq} 
\end{bmatrix} 
\end{center}


\subsubsection{Cross Entropy Minimization}



==> old_files.tex <==
% \[ \Delta M  = M_{i=1} - M_{i}  \] 
% \[ e_{c} = ( \lVert u_{t} \lVert^{2} + \rho )\tau + \Delta M  + h  \]



% Inequalities of the form (\ref{chance_const}) are known as chance constraints  \cite{chance_1}, \cite{chance_2} and are generally considered to be computationally intractable. Thus, existing works focuses on deriving tractable approximations of (\ref{chance_const}) under two predominant assumption. Firstly, the obstacles are assumed to have defined geometric shapes (e.g ellipsoid) and as a result it becomes possible to derive an analytical expression for $d(x(t), y(t))$. Second, the perception uncertainty are often assumed to be Gaussian. When both the assumptions are made simultaneously it even becomes possible to formulate a convex approximation of (\ref{chance_const}) \cite{chance_guassian}.

% Our work relaxes both the above mentioned assumptions substantially expanding the applicability of chance-constrained optimization based motion planning in real-world environment. We handle chance-constraints on collision avoidance by treating  $d(x(t), y(t))$ as a black-box model that can only be queried from a voxel-grid representation of the world. Secondly, we make no assumption on the underlying perception uncertainty.

% \noindent \textbf{Sample Average Approximation:} The most challenging part in handling chance constraints is estimating the distribution of the constraint function i.e the r.h.s of (\ref{chance_const}). Authors in \cite{saa} 


%  \begin{subequations} \label{CCO}
%  \begin{align}
%     E(C_{i}) = \sum_{ i=0 }^{N} \lambda_{1} MMD(C_{i}) + \lambda_{2} F_{a}(C_{i}) + \lambda_{3} \lVert C_{i-1} - 2C_{i} + C_{i+1} \lVert 
%  \end{align}
%     \begin{align}
%   \textrm{s.t.} \quad   P( (r_{safe} - d_{i } ) < 0 ) >  \eta   
%     \end{align}
%  \end{subequations}
 
%  \[  F_{a}(C_{i}) = ( a_{min} - a_{c_i} )(a_{max} - a_{c_i} ) \]
% Optimization of functions using constrains in the form of  \ref{CCO} is known as Chance Constrained Optimization (CCO). In general CCO has a high computational complexity that  stems from the presence of chance constrains, a  non linear function \textit{f(.)} and a large set of samples . In this section we reformulate this problem into a tractable non linear optimization problem.  \par

% Our solution is based on the theorems proposed in \cite{Reactive_navigation_RKHS}, where it states that MMD can act as a surrogate to the moment matching problem and decreasing the Maximum Mean Discrepancy (MMD) residual between the RKHS embedding of $\mathnormal{P_{f}}$ and desired distribution $\mathnormal{P_{f^{des}}}$, is a method to match the first \textit{d} moments between the distributions. 
% \begin{equation} \label{MMD}
% L_{dist}    = \lVert \mu_{P_{f}} - \mu_{P^{des}} \lVert^{2}  
% \end{equation}

% Equation \ref{MMD} can be further expanded to obtain 

% \begin{equation} \label{MMD_expand}
%     \lVert \mu - \mu_{des} \lVert ^{2} = \langle \boldsymbol{\mu_{P_{f}}} , \boldsymbol{ \mu_{P_{f}} }\rangle - 2 \langle \boldsymbol{ \mu_{P_{f}}}, \boldsymbol{\mu_{P^{des}}}  \rangle + \langle \boldsymbol{\mu_{P^{des}}}  , \boldsymbol{\mu_{P^{des}}}  \rangle 
% \end{equation}

% Equation \ref{MMD_expand} computes the inner product between the functions, that are linear combinations of kernel functions.  The use of the "kernel trick" allows for the computation of the inner product by pointwise computation of the kernel function. 


% \subsubsection{Desired Distribution}

% In general construction of an exact desired distribution is an intractable problem \cite{Reactive_navigation_RKHS} , therefore we propose a unique representation of the desired distribution as a dirac function. Furthermore, this representation provides attractive properties which leverages computational advantages. \par

% Consider a distance distribution $\mathnormal{Q}$ represented by samples \textit{$\Tilde{d_{i}}$}. The distribution can be considered ideal if all the samples in it are avoiding the obstacle i.e $\forall \Tilde{d_{i}} \in \mathnormal{Q}$, $r_{safe} -\Tilde{d_{i}} < 0 $.   \par

% \begin{equation} \label{dirac}
% f(d_{i}) = \max ( 0 , (r_{safe} - \Tilde{d_{i}} )) 
% \end{equation}
% \[ \forall \Tilde{d_{i}} \in \mathnormal{Q}\]

% Through equation \ref{dirac} where all samples are drawn from an ideal distribution we observe that $f(d_{i})$ is a set of zeros. {\color{blue}{\textbf{To be Continued}}}

% \begin{equation}
%      P(f(d)) \rightarrow \delta
% \end{equation}


The proposed MMD based front end path searching method is built upon the kinodynamic A* algorithm which was proposed in  \cite{FastPlanner}. It is a heuristic based planning procedure that searches a initial path in discretized control space.  The search loop is similar to that of that of the standard A* algorithm, where a open and closed set of voxels are maintained and instead of straight lines a motion primitive that obeys the quadrotor dynamics is used to represent the edge of the graph.  

Given the current state of the quadrotor and the control limits $[ -u_{max} , u_{max}]$, multiple control inputs for each axis is generated uniformly $ \{ -u_{max} , -\frac{r-1}{r} u_{max}, \hdots , \frac{r-1}{r} u_{max} , u_{max} \}$. This results in $(2r+1)^{3}$ motion primitives, which are applied iteratively to expand in the grid map. The \textit{Edge Cost} that connect two nodes for a given control input $u_{t}$ applied for time $\tau$ is given by 
is given by equation (\ref{edge_cost}), where $\Delta M$ is the difference between the MMD cost between the current node $n_i$ and the new node $n_{i+1}$ obtained after primitive expansion. 


 $\Delta M$ would have a lower value for primitives that guide the trajectory away from the obstacle and would be higher when the trajectory is moved towards an obstacle. 


If a path has \textit{n} motion primitives from the start state ($x_{s}$) to the current state ($x_{c}$)  the cost \textit{$g_{c}$} is calculated as $g_{c} = \sum _{i=0}^{n} ( \lVert u_{ti} \lVert^{2} + \rho )\tau + \Delta M_{(i,i+1)}$.  

An information heuristic is essential to compute an optimal trajectory in real time, the Pontryagins minimum principal \cite{pontagris_min_principal} is used to obtain the  close form minimal trajectory from current state ($x_{c}$) to the goal ($x_{g}$) and the roots of the optimal path is used to calculate the heuristic cost ($h_{c}$) as described in \cite{FastPlanner}. The cost $f_c$ is calculated as $ f_{c} = g_{c} + h_{c}$.

After the every iteration of primitive expansion, if the new nodes is in the same voxel they are pruned. The process continues until any one primitive reaches the goal or a direct, safe and feasible path exists between current state ($x_{c}$) and goal state ($x_{g}$). 



A number of methods were proposed in the last half a decade targeting navigation of UAV systems specific to quadrotors that include \cite{FastPlanner}  \cite{gao2017quadrotor} \cite{RAPPIDS} \cite{RAPTOR} \cite{Topo}. Many of these methods have also been implemented with compute available onboard the UAV systems. However none of these methods to the best of our knowledge model the uncertainty associated with sensor measurements and its concomitant effect on trajectory planning and execution

% \Madhav{fix latex error}

In this paper we propose a framework that models the non-parametric uncertainty associated with depth measurements seen in commodity hardware \cite{realsense}. This uncertainty is transformed to the uncertainty in voxel maps or octomaps. To make the grid world uncertainty amenable to a planning framework we compute thereof  the uncertainty distribution over the closest distance to an occupied voxel from a given freespace location in the map. We make use of this uncertainty distribution in the frontend planner that implements a Kinodynamic Astar with MMD cost as the guiding principle in selecting the best amongst the sampled trajectories that typically has the lowest MMD cost. The MMD cost is evaluated as the distance between two probability(uncertainty) distributions in the Reproducing Kernel Hilbert Space (RKHS). In our proposed framework the two distributions are the desired collision free distribution modeled as a Dirac Delta function and the uncertainty distribution over the closest occupied voxel from the current location. The backend planner is implemented as a Cross Entropy Method (CEM) optimization  \cite{iCEM} \cite{CEM1} that improves the smoothness and dynamic feasibility of the selected front end trajectory while continuing to be collision free. 

Specifically we claim the following contributions.
\begin{enumerate}[nolistsep]
    \item \textit{Uncertainty Aware Trajectory Planning Over Voxel Grids/Octomap:}  This paper shows for the first time a trajectory planning and navigation framework that accounts for voxel uncertainty accrued due to non-parametric sensor noise uncertainty. The benefits of the proposed framework is compared extensively with deterministic frameworks \cite{FastPlanner} and those that model uncertainty conservatively \cite{bounding1}. The benefits are seen in the form of almost negligible collisions under the duress of varying levels of sensor noise even as the deterministic framework reports high collision rates. Despite almost zero collision the trajectory maneuvers due to the proposed method are far less deviant in contrast with methods that grow the gridworld directly by the uncertainty in sensor measurement
    
    \item \textit{Realtime Onboard Implementation:} Exploiting the properties of the Kernel matrices as well as through learnt low dimensional representations of gridworld uncertainty we showcase near real-time performance in simulation and through an onboard implementation on commodity hardware \cite{Intel NUC}. 
    
    \item \textit{Novel Formulation of the Desired Distribution: } We show how the desired collision free distribution can be modeled as a Dirac Delta function that circumvents the need to compute a desired distribution on the fly by sampling from the space of controls \cite{Reactive_navigation_RKHS , CCO_RKHS} . This results in reduction in compute time for MMD cost and the eventual reduction in time taken to select the best frontend trajectory.
    
    \item \textit{Ablations:} We tabulate a variety of ablations that portrays the role for each part of the uncertainty modelling pipeline. These include the benefits of caching Kernel matrices and the encoder architecture that provides for a low dimensional rendering of the uncertainty distribution.
    
    \item \textit{Distribution and Obstacle Geometry Agnostic Uncertainty Models: } Unlike prior chance constrained approaches \cite{Mora_RAL2019, probabilistic_avoidance, Reactive_navigation_RKHS} to uncertainty aware collision avoidance the current formulation is both agnostic to obstacle geometry (discs, ellipses etc) and the nature of the uncertainty distribution (parametric like Gaussian).

    \end{enumerate}
    

\subsection{Trajectory and Motion Planning: } Trajectory and motion planning for quadrotor systems have long been studied in the literature. While some focus on trajectory generation as an optimization program \cite{min_snap, polynomial_trajectory, gao2017quadrotor} others integrate planning and navigation with perception \cite{Autonomous_exploration, Shen-2016}. 

Over the recent years voxel based or volumetric maps have emerged as a popular choice of representation over which trajectory plans are computed and executed \cite{FastPlanner, ewok , Topo, RAPTOR}. The popularity of such discretized voxel/volumetric maps initially introduced and disseminated through \cite{octomap}, stems in part due to their amenability to Signed Distance and Euclidean Signed Distance Field representations that are conveniently adopted by trajectory planning frameworks, all the more so by gradient based methods \cite{Topo, RAPTOR}.

\subsection{Uncertainty Incorporated Planning and Avoidance: } In parallel a number of works have modelled uncertainty in trajectory planning and collision avoidance. The earlier works tended to grow the obstacles by the uncertainty of the distribution \cite{ bounding1 , bounding2}  that resulted in conservative trajectories as exemplified in \cite{bounding_volume}. Later methods have resorted to chance constraint formulations within a robust MPC framework as their preferred choice. Chance constraint formulations are typically intractable with analytical expressions for such constraints being non-existent. Traditionally such constraints are replaced with smartly crafted surrogates that closely approximate the original constraints \cite{probabilistic_avoidance, bounding_volume,  IROS_15}. However a closed form expression for these constraints is only possible if the underlying random variables that make up the constraint expression belong to a Gaussian Distribution.

One of the first such methods that handled non parametric uncertainty in the context of collision avoidance, did so by incorporating a RKHS embedding of the moment matching function as a cost term within a robust MPC framework \cite{Reactive_navigation_RKHS, CCO_RKHS}. The RKHS framework originally proposed in \cite{BT_61} and adapted to a robotics setting through \cite{Reactive_navigation_RKHS, CCO_RKHS} is particularly attractive due to its distribution agnostic feature and low sample complexity. Other approaches include linearization techniques \cite{Mora_RAL2019} to retain the Gaussian property of the constraint function. Such formulations cannot handle situations where the random variables underlying the distribution are in themselves non-parametric.
It is to be noted that all the above approaches assume well defined robot/obstacle shapes such as discs, polygons that enable the constraint function to be tractable.

\subsection{Uncertainty Formulation over Voxel/Volumetric grids: } In contrast to above methods the current formulation poses the chance constraint optimization over a 3D voxel map built from noisy sensor data. There are no assumptions about the nature of the sensor noise nor the obstacle shape as the voxel occupancy values are a shape agnostic representation of the map. To the best of our knowledge this is the first such approach to handle non-parametric uncertainty underlying the voxel map distribution for a trajectory planning formulation.  

